What Would Trojans Do? Exploiting Partial-Information Vulnerabilities in Autonomous Vehicle Sensing

Safety-critical sensors in autonomous vehicles (AVs) form an essential part of the vehicle's trusted computing base (TCB), yet they are highly susceptible to attacks. Alarmingly, Tier 1 manufacturers have already exposed vulnerabilities to attacks introducing Trojans that can stealthily alter sensor outputs. We analyze the feasible capability and safety-critical outcomes of an attack on sensing at a cyber level. To further address these threats, we design realistic attacks in AV simulators and real-world datasets under two practical constraints: attackers (1) possess only partial information and (2) are constrained by data structures that maintain sensor integrity.Examining the role of camera and LiDAR in multi-sensor AVs, we find that attacks targeting only the camera have minimal safety impact due to the sensor fusion system's strong reliance on 3D data from LiDAR. This reliance makes LiDAR-based attacks especially detrimental to safety. To mitigate the vulnerabilities, we introduce security-aware sensor fusion incorporating (1) a probabilistic data-asymmetry monitor and (2) a scalable track-to-track fusion of 3D LiDAR and monocular detections (T2T-3DLM). We demonstrate that these methods significantly diminish attack success rate.

==> 90-acknowledgments.tex <==
\begin{acks}
...
\end{acks}

==> algorithms/alg_att_executer.tex <==
% --------------------------------------
\begin{algorithm}
    \caption{Execute: LiDAR-Level Execution Module}
    \label{alg:execute}
    \begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \REQUIRE Point cloud $PC$ of shape [n x 4], frame index $k\geq0$
    \ENSURE  Point cloud $PC$ of shape [n x 4]
    \STATE tbd
    \RETURN $PC$
    \end{algorithmic} 
\end{algorithm}
% --------------------------------------

==> algorithms/alg_att_monitoring.tex <==

% --------------------------------------
\begin{algorithm}
    \caption{Monitor: LiDAR-Level Monitoring Module}
    \label{alg:monitor}
    \begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \REQUIRE Point cloud $PC$ of shape [n x 4], frame index $k\geq0$
    \ENSURE T\_Lidar2Ground (T\_L2G), obj\_tracks
    \STATE T\_L2G, obj\_tracks $\leftarrow$ None
    \STATE UP $\leftarrow$ MonitorUp(PC, k) \COMMENT{Finds up axis and direction}
    \IF {found UP}
        \STATE PC\_BEV $\leftarrow$ ProjectToBEV(PC, UP) \COMMENT{Bird's eye view}
        \STATE FORWARD, LEFT $\leftarrow$ MonitorFwdLeft(PC\_BEV, k)
        \IF {found FORWARD}
            \STATE C $\leftarrow$ MakeCoordinate(FORWARD, LEFT, UP)
            \STATE obj\_tracks $\leftarrow$ DetectAndTrack(PC, C)
            \STATE G $\leftarrow$ EstimateGroundPlane(PC, C)
            \IF {found G}
                \STATE T\_L2G $\leftarrow$ MakeTransform(C, G)
            \ENDIF
        \ENDIF
    \ENDIF
    \RETURN T\_L2G, obj\_tracks
    \end{algorithmic} 
\end{algorithm}
% --------------------------------------

==> algorithms/alg_att_scheduler.tex <==

% --------------------------------------
\begin{algorithm}
    \caption{Schedule: LiDAR-Level Scheduling Module}
    \label{alg:schedule}
    \begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \REQUIRE T\_Lidar2Ground, obj\_tracks, frame index $k\geq0$
    \ENSURE att\_sched
    \STATE tbd
    \RETURN att\_sched
    \end{algorithmic} 
\end{algorithm}
% --------------------------------------

==> algorithms/alg_coordinate_monitor.tex <==
% --------------------------------------
\begin{algorithm}
    \caption{LiDAR-Level Cyber Coordinate Monitoring}
    \begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \REQUIRE Point cloud $PC$ of shape [n x 4], frame index $k\geq0$
    \ENSURE  Point cloud $PC$ of shape [n x 4]
    \\ \textit{Initialize:}  \COMMENT{``None" evals to false}
    \IF {k == 0}
    \STATE axis, parity $\leftarrow$ dict(up:FIFO$(n_1)$, forward:FIFO$(n_2)$)
    \STATE DMAP $\leftarrow$ dict(0:`x', 1:`y', 2:`z')
    \STATE SMAP $\leftarrow$ dict(-1:`-', +1:`+')
    \STATE found $\leftarrow$ dict(forward:None, up:None)
    \STATE tracker $\leftarrow$ Multi-object 2D tracker
    \STATE track\_history $\leftarrow$ FIFO$(n_3)$
    \ENDIF
    \\ \textit{Coordinate Monitor:} 
    \IF {not found[up]}
    % \COMMENT{Up Direction}
    \STATE axis[up].push( $\argmin \ \sigma(PC,\ \text{axis}=0)$ )
    \STATE parity[up].push( $\sign\left(\mu(PC[:,\, \text{axis}_{\text{up/down}}[k]]\right)$ )
    \IF {$k\geq n_1$}
    \STATE updir, counts = mode $\left(\text{parity[up]}\oplus \text{axis[up]}\right)$
    \IF {$\sfrac{\text{counts}}{\text{len(axis[up])}} > \tau_1$}
        \STATE found[up] = SMAP[updir[0]] + DMAP[updir[1]] \COMMENT{e.g., ``+z"}
    \ENDIF
    \ENDIF
    \ELSE
    % \COMMENT{Forward Direction}
    \STATE $\text{PC}_{\text{BEV}} \leftarrow$ PC[:, !found[up]]
    \STATE clusters $\leftarrow$ DBSCAN($\text{PC}_{\text{BEV}}$)
    \STATE clusters $\leftarrow$ filter(clusters) \COMMENT{Filter out illogical clusters}
    \STATE tracks $\leftarrow$ tracker.track(clusters)
    \STATE track\_history.push(tracks)
    \ENDIF
    \STATE Buffer k frames
    \\ \quad \textit{Ground Plane Monitor}
    \\ \quad \textit{Ground Plane Monitor}
    \FOR {$i = l-2$ to $0$}
    \STATE statements..
    \IF {($i \ne 0$)}
    \STATE statement..
    \ENDIF
    \ENDFOR
    \RETURN $P$ 
    \end{algorithmic} 
\end{algorithm}
% --------------------------------------

==> figures/figure_av_attack_surfaces.tex <==
% ============================
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{diagrams/av-cyber-attack-surfaces.drawio.pdf}
    \caption{A general case where \emph{any} AV substrate(s) may be compromised. Unlike spoofing to compromise sensing (blue) or white-box attacks on perception, cyber threat models consider that any processing or communication platform (red) could be compromised in the AV chain.}
    \label{fig:av-attack-surfaces}
\end{figure}
% ============================

==> figures/figure_av_attack_vectors.tex <==
% ============================
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.6\linewidth]{diagrams/av-cyber-attack-vectors.drawio.pdf}
    \caption{Diverse connected components in AVs present new and yet under-studied attack vectors for cyber-based threats.}
    \label{fig:av-attack-vectors}
\end{figure}
% ============================

==> figures/figure_security_metrics.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{diagrams/diagram-3-analysis.png}
    \caption{Analysis needed at multiple levels of the AV stack. Perception, tracking, and prediction can use longitudinal datasets; planning \& control need AV simulator or real AV.}
    \label{fig:av-attack-analysis}
\end{figure}

==> tables/table_attack_models.tex <==

% ----------------------
\begin{table}[!t]
\centering
\begin{tabular}{||l l c c c||} 
 \hline
 Strategy & Intent & Monitor & Schedule & Execute \\ [0.5ex] 
 \hline\hline
 Naive & Brake & C, GP & S, B & A \\ 
 \hline
 Naive & Drift & C, GP & S, D & A \\
 \hline
 Frustum & Brake & C, GP, O & S, B & A \\
 \hline
 Frust. & Takeover & C, GP, O & S, A & A/M \\
 \hline
 Frust. & Drift & C, GP, O & S, D & A \\
 \hline
\end{tabular}
\caption{Attack models evaluated under longitudinal scenarios and description of active modules for each attack.\\ \textit{Monitor} -- C=Coordinate, GP=Ground plane, O=Objects. \\ \textit{Schedule} -- S=Stable, A=Accelerate, B=Brake, D=Drift.\\ \textit{Execute} -- A=Add, M=Move, R=Remove.}
\label{table:attack-models}
\end{table}
% ----------------------

==> tables/table_attack_reviews.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|l}
        Attack & Threat Model & Attacker's Knowledge & Demonstrated Capability & Assumed Capability \\
        \hline \hline
        AdvLiDAR~\cite{2019cao-spoofing} & Spoofing & White-Box & Insert 60 points & Precise laser aiming w/ white-box. \\
        BlackBox~\cite{2020sun-spoofing} & Spoofing & Black-Box & Insert 200 points & Precise laser aiming in pattern of a car. \\
        Frustum~\cite{2022hally-frustum} & Spoofing & Black-Box & Insert 200 points & Precise laser aiming. \\
        AdvRoof~\cite{2020tuphysicalatt} & Physical Adv. Object & White-Box & Gradient-based adv. object & White-box model access, large adv. obj.\\
        MSF-Adv~\cite{2021invisiblecamlidar} & Physical Adv. Object & White-Box & Gradient-based adv. object & White-box model access.\\
        DirtyRoad~\cite{2021dirtyroad} & Physical Adv. Object & White-Box & Gradient-based dav. object & White-box model access.\\
        \hline
        \tworowsubtablecenter{Cyber Attack}{(this work)} & \tworowsubtablecenter{Malware on Sensor, Comms,}{or Processing substrate} & \tworowsubtablecenter{Incoming LiDAR}{point cloud only} & \tworowsubtablecenter{Deriving situational awareness}{from point cloud online} & \tworowsubtablecenter{Computational and}{memory capability}\\
        \hline
    \end{tabular}
    }
    \caption{Existing state of the art attacks (top) fall into spoofing and physical-adversarial object categories with white and black-box flavors. All require either precise laser aiming or white-box model access. Ours (bottom) is the first to consider an increasingly-likely cyber threat model with nearly no information about the system and the environment of the vehicle.}
    \label{tab:attack-review}
\end{table*}

==> tables/table_results_case_studies.tex <==
% ============
\begin{table*}[!t]
    \centering

\begin{tabular}{lllll}
\toprule
                                                                      AV Case &                                Attacker &                                                                  Percep. Outcomes &                                                                        Track Outcomes &                                                   Safety Outcomes \\ \midrule
\midrule
                                                    \ref{av:lidar} Lidar-Only &             \ref{att:fp} False Positive &         \tworowsubtableleft{K -- FP:  149, FN: \,  79}{N -- FP: \,  17, FN:  292} &   \tworowsubtableleft{K -- FT: \,  64, MT: \, \,  0}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  4}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (1)} &             \ref{att:fp} False Positive &         \tworowsubtableleft{K -- FP:  149, FN: \,  79}{N -- FP: \,  19, FN:  292} &   \tworowsubtableleft{K -- FT: \, \,  0, MT: \, \,  0}{N -- FT: \, \,  8, MT: \,  -5} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (2)} &             \ref{att:fp} False Positive &         \tworowsubtableleft{K -- FP:  149, FN: \,  79}{N -- FP: \,  19, FN:  292} &   \tworowsubtableleft{K -- FT: \, \,  0, MT: \, \,  0}{N -- FT: \, \,  2, MT: \,  -2} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
           \ref{av:ttt} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Tracking} &             \ref{att:fp} False Positive &         \tworowsubtableleft{K -- FP:  149, FN: \,  79}{N -- FP: \,  19, FN:  292} & \tworowsubtableleft{K -- FT: \, \,  0, MT: \, \,  0}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
                                                    \ref{av:lidar} Lidar-Only &      \ref{att:forreplay} Forward Replay &             \tworowsubtableleft{K -- FP:  316, FN:  127}{N -- FP:  147, FN:  117} &           \tworowsubtableleft{K -- FT:  144, MT:  113}{N -- FT: \, \,  4, MT: \,  30} & \tworowsubtableleft{K -- Unsafe: \, \,  1}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (1)} &      \ref{att:forreplay} Forward Replay &             \tworowsubtableleft{K -- FP:  316, FN:  127}{N -- FP:  147, FN:  117} &         \tworowsubtableleft{K -- FT:  173, MT: \,  88}{N -- FT: \, \,  0, MT: \,  44} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (2)} &      \ref{att:forreplay} Forward Replay &             \tworowsubtableleft{K -- FP:  316, FN:  127}{N -- FP:  147, FN:  117} &             \tworowsubtableleft{K -- FT: \,  43, MT:  111}{N -- FT:  -13, MT: \,  30} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  9} \\ \midrule
           \ref{av:ttt} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Tracking} &      \ref{att:forreplay} Forward Replay &             \tworowsubtableleft{K -- FP:  316, FN:  127}{N -- FP:  147, FN:  117} &       \tworowsubtableleft{K -- FT: \, \,  0, MT: \,  88}{N -- FT: \,  -3, MT: \,  18} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
                                                    \ref{av:lidar} Lidar-Only &      \ref{att:revreplay} Reverse Replay &             \tworowsubtableleft{K -- FP:  313, FN:  115}{N -- FP:  150, FN:  114} &           \tworowsubtableleft{K -- FT:  144, MT:  103}{N -- FT: \, \,  2, MT: \,  28} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (1)} &      \ref{att:revreplay} Reverse Replay &             \tworowsubtableleft{K -- FP:  313, FN:  115}{N -- FP:  150, FN:  114} &             \tworowsubtableleft{K -- FT:  113, MT:  106}{N -- FT: \,  42, MT: \,  37} & \tworowsubtableleft{K -- Unsafe: \, \,  4}{N -- Unsafe: \, \,  5} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (2)} &      \ref{att:revreplay} Reverse Replay &             \tworowsubtableleft{K -- FP:  313, FN:  115}{N -- FP:  150, FN:  114} &             \tworowsubtableleft{K -- FT: \,  18, MT:  103}{N -- FT:  -24, MT: \,  32} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
           \ref{av:ttt} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Tracking} &      \ref{att:revreplay} Reverse Replay &             \tworowsubtableleft{K -- FP:  313, FN:  115}{N -- FP:  150, FN:  114} &       \tworowsubtableleft{K -- FT: \, \,  0, MT: \,  81}{N -- FT: \,  -3, MT: \,  17} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
                                                    \ref{av:lidar} Lidar-Only &         \ref{att:remove} Object Removal & \tworowsubtableleft{K -- FP: \,  97, FN: \,  35}{N -- FP: \, \,  0, FN: \, \,  0} &   \tworowsubtableleft{K -- FT: \, \,  0, MT: \,  32}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (1)} &         \ref{att:remove} Object Removal & \tworowsubtableleft{K -- FP: \,  97, FN: \,  35}{N -- FP: \, \,  0, FN: \, \,  0} & \tworowsubtableleft{K -- FT: \, \,  7, MT: \, \,  7}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (2)} &         \ref{att:remove} Object Removal & \tworowsubtableleft{K -- FP: \,  97, FN: \,  35}{N -- FP: \, \,  0, FN: \, \,  0} &   \tworowsubtableleft{K -- FT: \, \,  0, MT: \,  25}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
           \ref{av:ttt} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Tracking} &         \ref{att:remove} Object Removal & \tworowsubtableleft{K -- FP: \,  97, FN: \,  35}{N -- FP: \, \,  0, FN: \, \,  0} &   \tworowsubtableleft{K -- FT: \, \,  0, MT: \,  29}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
                                                    \ref{av:lidar} Lidar-Only & \ref{att:frust-trans} Frustum Translate &   \tworowsubtableleft{K -- FP:  142, FN: \,  50}{N -- FP: \, \,  0, FN: \, \,  0} &     \tworowsubtableleft{K -- FT: \,  45, MT: \,  47}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  8}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (1)} & \ref{att:frust-trans} Frustum Translate &   \tworowsubtableleft{K -- FP:  142, FN: \,  50}{N -- FP: \, \,  0, FN: \, \,  0} &     \tworowsubtableleft{K -- FT: \,  70, MT: \,  21}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  8}{N -- Unsafe: \, \,  0} \\ \midrule
\ref{av:cam-lidar} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Detection (2)} & \ref{att:frust-trans} Frustum Translate &   \tworowsubtableleft{K -- FP:  142, FN: \,  50}{N -- FP: \, \,  0, FN: \, \,  0} &     \tworowsubtableleft{K -- FT: \,  32, MT: \,  45}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
           \ref{av:ttt} \tworowsubtablecenter{Cam-LiDAR Fusion}{ at Tracking} & \ref{att:frust-trans} Frustum Translate &   \tworowsubtableleft{K -- FP:  142, FN: \,  50}{N -- FP: \, \,  0, FN: \, \,  0} &   \tworowsubtableleft{K -- FT: \, \,  0, MT: \,  47}{N -- FT: \, \,  0, MT: \, \,  0} & \tworowsubtableleft{K -- Unsafe: \, \,  0}{N -- Unsafe: \, \,  0} \\ \midrule
\bottomrule
\end{tabular}

\caption{Attacker can execute multiple attacks in a cyber context with only access to the LiDAR sensor data. Several attacks satisfy the 3 necessary conditions for high attack impact. Attacker sets parameters a-priori for executing over longitudinal sequence since he has no prior scene knowledge (see Appendix~\ref{appendix:case-study-details}).}
\label{table:results_case_studies}
\end{table*}
% ============

% Number of unsafe frames varies between data sources due to difference in framerates of KITTI (10 Hz) and nuScenes (2 Hz).$^\dagger$Frustum attack starts at increased distance compared to naive attack and uses "stable" and "attacking" stages, so number of unsafe frames expected to be lower than total attacked frames.
